Encrypted Data Processing

In this paper, we present a comprehensive architecture for confidential computing, which we show to be general purpose and quite efficient. It executes the application as is, without any added burden or discipline requirements from the application developers. Furthermore, it does not require the trust of system software at the computing server and does not impose any added burden on the communication subsystem. The proposed Encrypted Data Processing (EDAP) architecture accomplishes confidentiality, authenticity, and freshness of the key-based cryptographic data protection by adopting data encryption with a multi-level key protection scheme. It guarantees that the user data is visible only in non-privileged mode to a designated program trusted by the data owner on a designated hardware, thus protecting the data from an untrusted hardware, hypervisor, OS, or other users' applications. The cryptographic keys and protocols used for achieving these confidential computing requirements are described in a use case example. Encrypting and decrypting data in an EDAP-enabled processor can lead to performance degradation as it adds cycle time to the overall execution. However, our simulation result shows that the slowdown is only 6% on average across a collection of commercial workloads when the data encryption engine is placed between the L1 and L2 cache. We demonstrate that the EDAP architecture is valuable and practicable in the modern cloud environment for confidential computing. EDAP delivers a zero trust model of computing where the user software does not trust system software and vice versa.

==> texSections/Analysis.tex <==
\label{Analysis}

To gain a better understanding of the performance impact of data encryption and data decryption overhead in an EDAP-enabled system, we built two different performance models – an analytical model and a cycle accurate timing model.  The analytical model provides an upper bound estimation in performance degradation with minimal hardware addition of a single data encryption engine.  It also offers insights in processor performance sensitivity to the latency of data encryption engine and the frequencies of its usage.  The cycle accurate timing model delivers a more comprehensive performance evaluation of different EDAP implementations in a modern superscalar processor architecture.  

==> texSections/Architecture.tex <==
\label{Architecture} 
In \cite{LaurenBiernacki}, Biernacki \etal propose approach to encrypted data processing where ciphertext is decrypted as the last step just before a functional unit performs an operation using it as an input, and the result produced by the functional unit is encrypted back as the first step after the functional unit produces the result.  The data remains encrypted when in the register files.  However, decrypting and encrypting the ciphertext for each instruction increase the execution latency significantly with adverse impact on overall performance.  An important requirement not addressed in this work is restricting an adversaries application from accessing DO's data, \ie allowing access to DA's data to AA's applications, where AA's application has been authenticate to PP by the DO as described in section \ref{Protocol}.  By confining cyphertext to a minimal section of processor hardware, just the functional unit, the processor design can be verified rigorously for security.

Our approach to encrypted data processing is similar to \cite{LaurenBiernacki}.
The cleartext is confined to a small section of the processor hardware.  However, we propose to share the cleartext across instructions in a designated user application.  
This avoids the encryption-decryption latency, without exposing the data to any software other than the designated application.  In particular, the system software that runs at higher privilege levels in a user's application, untrusted per our thread model described in section \ref{ThreatModel}, too cannot access the cleartext of DO's protected data.  
	
The above mentioned cleartext buffering can be implemented in two ways.
The first is to 
store the cleartext in the register file shared by all functional units, but restricted access to the cleartext to a specific user application in problem-state only. The semantics of the load and store instructions are modified to make the load instructions decrypt the data before writing to the register file and the store instructions encrypt the data before storing back through the memory subsystem. \textit{Since only the problem-state of the corresponding program has access to the cleartext in the register file, two privilege instructions are created for the hypervisor to load and save program states.}  The second approach is to save/cache cleartext in the functional units of the processor in buffers which behave like caches, reducing the amount of hardware needed for moderate number of functional units.
We will refer to these two approaches as the Common Cleartext Approach and the Replicated Cleartext Approach.

Independent of where the cleartext resides, a second design consideration is to identify which data in memory is cyphertext and which is cleartext.  A naive solution is to assume that all the data is cyphertext in the application.  
The other solution is to either tag the cyphertext, such tag being inherited from the program inputs as described in \cite{SuhInfoFlowTracking}, or tag the instructions that are accessing cyphertext, so that the cyphertext can be decrypted before an operation is performed on it.

Bind to a thread:

Compare the two approaches - ease of implementaion vs. security risk.
	
	

==> texSections/CleartextLocalBuffer.tex <==
\label{CleartextLocalBuffer}

The Cleartext Local Buffer (CLB) design adds a local buffer to each of the functional units to store the cleartext of its recently accessed registers to allow the same application to bypass the data decryption of these cached values as shown in figure [?].  The data remain encrypted in the register file as in the baseline EDAP architecture.  However, the cleartext of a subset of the registers are stored in the CLB that is private to each functional unit.  To protects the cleartext data, each entry of the CLB is accessible to only a single authorized application in the user mode and not to other software.  This scheme is completely transparent to the software and the data is protected throughout the system. 
If the data is found within the CLB, the instruction bypasses the data decryption stage of the pipeline and the cleartext of its result is stored to the CLB through the write back bypass (WBI) while being encrypted (ENC) before written to the register file (WB) as shown in Figure [?].  The CLB resides within the functional unit and is a content addressable as a cache for encrypted entries of the register file, tagged with physical register numbers.  Furthermore, there is a snoop bus connected to each CLB to erase the entries when the register is reallocated as shown in Figure [?].  



==> texSections/CleartextProcessorCore.tex <==
\label{ClearProcessorCore}

\subsubsection{Memory Initialization}
dcbie, dcba, dcbr, dcbs


==> texSections/CleartextRegisterFile.tex <==
\label{CleartextRegisterFile}
The cleartext register file design decouples the data decryption, instruction execution, result encryption, and its writeback to register file in EDAP architecture to reduce its runtime and power consumption while preserving the data protection throughout the system.  Each data is decrypted immediately after it is read from the memory to the register file and each data is encrypted right before it is written from the register file back to the memory, as shown in Figure[?].  This scheme minimizes the number of time that a data needs to be decrypted and encrypted in EDAP.  To prevent the unencrypted data being read by other code or programs throughout the system, the Cleartext Register File design restricts the register access to only its user thread.  Since only the user application has access to its cleartext registers in user mode, new instructions are needed for the privilege programs, such as hypervisor and interrupt handlers, to save and to restore the its program states.
Section [?] shows the potential performance benefits of cleartext register file by comparing its pipeline structure with baseline EDAP design and describes the modified load and store semantics to keep cleartext data in the register file.  Section [?] introduces the protection tag in the register file to differentiate confidential and non-confidential data.  Section [?] presents the two privilege instructions, “load-and-hide” and “store-and-clear”, that are intended for the hypervisor code to load and store registers for context switching. 

\subsubsection{EDAP Pipeline with Cleartext Register File}

In a classic five stage RISC pipeline, there are instruction fetch (IF), instruction decode (ID), execute (EX), memory access (MEM), and register write back (WB) as shown in Figure [?].  Since the data are encrypted throughout the memory system in the EDAP architecture, we need to extend the pipeline with additional two stages to decrypt (DEC) the register value before the execute stage and encrypt (ENC) the result before the register write back as shown in Figure [?].  Decrypting and encrypting data of each instruction adds cycles to the overall execution and can significantly slow down the overall performance.  To reduce the decryption and encryption overhead, we allow the data to be stored as cleartext in the register file and its access is restricted to only the user application.  The data from the memory are decrypted before entering register file and the data are encrypted before written back to the memory.  Figure [?] shows the pipeline for non-memory instructions, load instructions, and store instructions for the EDAP architecture with cleartext register file implementation.  There are no extra cycles added for executing non-memory instructions because the data is already stored as cleartext in the register file as the baseline architecture.  After the encrypted data load from the memory, it is decrypted in DEC stage to produce cleartext for the register file.  Similarly, the cleartext data is encrypted in the ENC stage before storing it to the memory.  

\subsubsection{Protection Tag}

To provide different levels of data protection in the EDAP, we add a protection tag to each register in the register file to distinguish between data that is protected under EDAP and data that is not protected.   When the register is written by an instruction, its tag is set to protected if either it is a load instruction or one of the instruction’s source registers is set as protected.  If the register is tagged as protected, its data is only available to the problem state of the corresponding processor thread and it is encrypted before being stored to the memory.  Additionally, the protected register is erased at context switch or when the data is no longer needed.  

\subsubsection{Load-and-Hide and Store-and-Clear Instructions}

In EDAP architecture, only the user application can access its cleartext registers and this prevents revealing the cleartext data to other programs or code.  Two new privilege instructions, Load-and-Hide and Store-and-Clear, are added to the EDAP architecture to enable other codes, such as hypervisor and interrupts handlers, to save and restore the state of user application as needed.  The Load-and-Hide instruction restores the thread state by first loading the encrypted data from the memory, decrypting the data into cleartext, storing it into the register and hiding it from all codes that are not the designated user thread.  The Store-and-Clear instruction saves the thread state by first encrypting the cleartext register data, storing the cyphertext to the memory, and clearing the cleartext register from the register file.  These two instructions provide a safe way for other codes to interact with the user application without exposing its data and its encryption keys.   


==> texSections/FHE_Lite_Model.tex <==
%\newcommand{\quotient}[2]{\raisebox{0.2em}{$#1$}\left/\raisebox{-0.2em}{$#2$} \right.}
%\newcommand{\vbf}[1]{\bf$\mathcal{#1}$}
%\newcounter{savenumbering}

%I decided to put a very elemental model to see the
%structure of dependencies on the $k$ and $m$ from my original note. Now that Eknath has changed the M1 to 
%ingest these parameters and act on it, we can see the result {\it vis a vis} this model. Also we can use %it to 
%study the use of instruction fusion (that Gianfranco, Jessica, Eknath and I discussed today per Jessica's suggestion).
%First I define a set of variables, that I will use in deriving the model.

This is a very elemental analytical model for a EDAP implementation where the data encryption engine is placed within the functional unit enclave without any caching.  Therefore, extra cycle time is added to each data read from register file and each data write to register file.  Additionally, the data encryption unit is not pipelined and can only process one request at a time.  The major variables of the model are the number of instructions that use the data encryption engine to encrypt and decrypt data in EDAP architecture, the speed of data encryption engine, and the execution throughput of the program.

\subsubsection{Symbols}
Let base system denotes the system without any of the EDAP functions, and
prime system denotes the system with EDAP-enabled functional units.
\begin{eqnarray}
n &= &  \textrm{Number of instructions being executed}   \nonumber \\
n_f &=& \textrm{Number of instrctions for the architected functional units} \nonumber \\
n_m &=& \textrm{Number of instrctions for the memory sub-systems and others } \nonumber \\
\Rightarrow n &=& n_f + n_m \nonumber \\
C &=& \textrm{Total cycles taken to execute all the $n$ instructions in the base system } \nonumber \\
C'  &=& \textrm{Total cycles taken to execute all the $n$ instructions in the EDAP system } \nonumber \\
CPI &=& \textrm{Cycle Per Instruction (CPI) for the execution in the base system i.e. $C = n \; CPI$ } \nonumber \\
CPI_f &=& \textrm{Cycle Per Instruction (CPI) fo the functional units in the base system}  \nonumber \\
CPI_m &=& \textrm{Cycle Per Instruction (CPI) for the memory sub-system for the base system} \nonumber \\
x &=& \textrm{Fractions of functional unit instructions handling EDAP data. This is equal to $\frac{1}{m}$ } \nonumber \\
k &=& \textrm{added cycles by functional units for handling EDAP operations}
\end{eqnarray}

Note that $CPI_f$ and $CPI_m$ must satisfy

\begin{equation}
n CPI = (n_f + n_m) CPI = n_f * CPI_f + n_m *CPI_m
\end{equation}

In absence of any additional measurements, one can take these two quantities to be equal to $CPI$.

\subsubsection{Derived quantities}
\begin{eqnarray}
C &=& n \; CPI \nonumber \\
   &=& (n_f + n_m) CPI  \nonumber \\
C' &=& CPI_f \; n_f  \; (1-x) + (CPI_f  + k) \; n_f  \; x + CPI_m\; n_m \nonumber \\
     &=& CPI_f \; n_f  +  n_f  \; k x + CPI_m\; n_m \nonumber \\
\Rightarrow \frac{CPI'}{CPI} &=& \frac{CPI_f \; n_f  +  n_f  \; kx + CPI_m\; n_m } {n \; CPI } \nonumber \\
\frac{CPI'}{CPI} &=& 1 +  \frac{n_f  \; kx} {n \; CPI } \nonumber \\
CPI' &=& CPI +  \left ( \frac{n_f } {n } \right )   k\; x 
\end{eqnarray}

From this expression, one can see that the $\frac{CPI'}{CPI}$ is linear functions of $kx$ with an intercept (as expected) of one. The slope is $\frac{n_f}{n  CPI }$.  The $CPI'$ one gets out cycle accurate simulator, is likely to be different, as the above model is for an in-order machine and averages the details.  Thus due to finiteness of various queues, the $\frac{CPI'}{CPI}$ could be bigger than one, and due to the out of order nature of a processor, if present, it would less than one. The interplay between these two competing effects will yield the actual slowdown ration, but the model gives a ballpark range.

Assuming $\frac{n_f}{n}$ is 0.7, Figure \ref{fig:AnalyticalModelCPI} shows how the program runtime multiplies as we increase $kx$ value for different $CPI$ value.  As expected, the overhead of data decryption and encryption requirement in EDAP design slowdowns the cases with faster execution more rapidly.  Even with just $CPI$ of 1, our analytical model shows that the execution time doubles with $kx$ value of only 1.5.  The performance degradation is significant in this simple implementation. 

\begin{figure}
  \includegraphics[scale=.8]{figures/AnalyticalModelCPI.png}
  \caption{$\frac{CPI'}{CPI}$ plot as a function of $kx$ and $CPI$}
  \label{fig:AnalyticalModelCPI}
\end{figure}
